Who are the arbitrageurs? Empirical evidence from Bitcoin traders in the Mt. Gox exchange platform

We mine the leaked history of trades on Mt. Gox, the dominant Bitcoin exchange from 2011 to early 2014, to detect the triangular arbitrage activity conducted within the platform. The availability of user identifiers per trade allows us to focus on the historical record of 440 investors, detected as arbitrageurs, and consequently to describe their trading behavior. We begin by showing that a considerable difference appears between arbitrageurs when indicators of their expertise are taken into account. In particular, we distinguish between those who conducted arbitrage in a single or in multiple markets: using this element as a proxy for trade ability, we find that arbitrage actions performed by expert users are on average non-profitable when transaction costs are accounted for, while skilled investors conduct arbitrage at a positive and statistically significant premium. Next, we show that specific trading strategies, such as splitting orders or conducting arbitrage non aggressively, are further indicators of expertise that increase the profitability of arbitrage. Most importantly, we exploit within-user (across hours and markets) variation and document that expert users make profits on arbitrage by reacting quickly to plausible exogenous variations on the official exchange rates. We present further evidence that such differences are chiefly due to a better ability of the latter in incorporating information, both on the transactions costs and on the exchange rates volatility, eventually resulting in a better timing choice at small time scale intervals. Our results support the hypothesis that arbitrageurs are few and sophisticated users.

==> immagini/tikz/tikz-log-price.tex <==
\draw
(10.625,-0.114)--
(10.633,-0.176)--
(10.641,-0.18)--
(10.649,-0.177)--
(10.658,-0.188)--
(10.666,-0.188)--
(10.674,-0.213)--
(10.682,-0.209)--
(10.69,-0.208)--
(10.699,-0.208)--
(10.707,-0.208)--
(10.715,-0.203)--
(10.723,-0.202)--
(10.732,-0.205)--
(10.74,-0.203)--
(10.748,-0.208)--
(10.756,-0.208)--
(10.764,-0.195)--
(10.773,0.079)--
(10.781,-0.022)--
(10.789,0.037)--
(10.797,0.01)--
(10.805,0.029)--
(10.814,0.176)--
(10.822,0.279)--
(10.83,0.299)--
(10.838,0.439)--
(10.847,0.462)--
(10.855,0.527)--
(10.863,0.4)--
(10.871,0.451)--
(10.879,0.462)--
(10.888,0.462)--
(10.896,0.452)--
(10.904,0.454)--
(10.912,0.439)--
(10.921,0.407)--
(10.929,0.352)--
(10.937,0.378)--
(10.945,0.358)--
(10.953,0.392)--
(10.962,0.396)--
(10.97,0.43)--
(10.978,0.398)--
(10.986,0.423)--
(10.995,0.477)--
(11.003,0.477)--
(11.011,0.476)--
(11.019,0.509)--
(11.027,0.517)--
(11.036,0.653)--
(11.044,0.602)--
(11.052,0.565)--
(11.06,0.648)--
(11.068,0.628)--
(11.077,0.649)--
(11.085,0.978)--
(11.093,0.944)--
(11.101,0.957)--
(11.11,1.041)--
(11.118,1.033)--
(11.126,1.021)--
(11.134,1.009)--
(11.142,0.939)--
(11.151,1)--
(11.159,0.977)--
(11.167,0.973)--
(11.175,0.959)--
(11.184,0.946)--
(11.192,0.964)--
(11.2,0.954)--
(11.208,0.93)--
(11.216,0.897)--
(11.225,0.954)--
(11.233,0.952)--
(11.241,0.9)--
(11.249,0.901)--
(11.258,0.851)--
(11.266,0.903)--
(11.274,0.893)--
(11.282,0.973)--
(11.29,1.035)--
(11.299,1.078)--
(11.307,1.19)--
(11.315,1.238)--
(11.323,1.431)--
(11.332,1.543)--
(11.34,1.544)--
(11.348,1.591)--
(11.356,1.783)--
(11.364,1.949)--
(11.373,1.924)--
(11.381,1.851)--
(11.389,1.872)--
(11.397,1.97)--
(11.405,1.929)--
(11.414,1.973)--
(11.422,2.241)--
(11.43,2.28)--
(11.438,2.544)--
(11.447,2.389)--
(11.455,2.3)--
(11.463,2.276)--
(11.471,2.178)--
(11.479,2.246)--
(11.488,2.244)--
(11.496,2.23)--
(11.504,2.2)--
(11.512,2.211)--
(11.521,2.195)--
(11.529,2.151)--
(11.537,2.149)--
(11.545,2.167)--
(11.553,2.144)--
(11.562,2.168)--
(11.57,2.146)--
(11.578,2.173)--
(11.586,2.117)--
(11.595,2.041)--
(11.603,2.083)--
(11.611,1.995)--
(11.619,2.075)--
(11.627,2.067)--
(11.636,2.064)--
(11.644,2.057)--
(11.652,1.96)--
(11.66,1.961)--
(11.668,1.929)--
(11.677,1.928)--
(11.685,1.864)--
(11.693,1.869)--
(11.701,1.777)--
(11.71,1.701)--
(11.718,1.832)--
(11.726,1.756)--
(11.734,1.737)--
(11.742,1.682)--
(11.751,1.713)--
(11.759,1.701)--
(11.767,1.662)--
(11.775,1.617)--
(11.784,1.614)--
(11.792,1.575)--
(11.8,1.384)--
(11.808,1.526)--
(11.816,1.459)--
(11.825,1.583)--
(11.833,1.525)--
(11.841,1.508)--
(11.849,1.481)--
(11.858,1.477)--
(11.866,1.491)--
(11.874,1.415)--
(11.882,1.362)--
(11.89,1.371)--
(11.899,1.408)--
(11.907,1.405)--
(11.915,1.497)--
(11.923,1.476)--
(11.932,1.489)--
(11.94,1.483)--
(11.948,1.519)--
(11.956,1.509)--
(11.964,1.568)--
(11.973,1.601)--
(11.981,1.642)--
(11.989,1.622)--
(11.997,1.699)--
(12.005,1.723)--
(12.014,1.859)--
(12.022,1.857)--
(12.03,1.845)--
(12.038,1.844)--
(12.047,1.842)--
(12.055,1.816)--
(12.063,1.814)--
(12.071,1.755)--
(12.079,1.748)--
(12.088,1.792)--
(12.096,1.775)--
(12.104,1.767)--
(12.112,1.778)--
(12.121,1.748)--
(12.129,1.679)--
(12.137,1.655)--
(12.145,1.692)--
(12.153,1.699)--
(12.162,1.69)--
(12.17,1.679)--
(12.178,1.703)--
(12.186,1.695)--
(12.195,1.695)--
(12.203,1.736)--
(12.211,1.731)--
(12.219,1.688)--
(12.227,1.677)--
(12.236,1.676)--
(12.244,1.684)--
(12.252,1.706)--
(12.26,1.694)--
(12.268,1.681)--
(12.277,1.69)--
(12.285,1.702)--
(12.293,1.701)--
(12.301,1.713)--
(12.31,1.718)--
(12.318,1.714)--
(12.326,1.701)--
(12.334,1.714)--
(12.342,1.712)--
(12.351,1.708)--
(12.359,1.702)--
(12.367,1.702)--
(12.375,1.71)--
(12.384,1.712)--
(12.392,1.713)--
(12.4,1.712)--
(12.408,1.713)--
(12.416,1.722)--
(12.425,1.723)--
(12.433,1.743)--
(12.441,1.75)--
(12.449,1.775)--
(12.458,1.819)--
(12.466,1.815)--
(12.474,1.832)--
(12.482,1.81)--
(12.49,1.824)--
(12.499,1.826)--
(12.507,1.816)--
(12.515,1.829)--
(12.523,1.86)--
(12.532,1.898)--
(12.54,1.919)--
(12.548,1.967)--
(12.556,1.954)--
(12.564,1.943)--
(12.573,1.951)--
(12.581,1.975)--
(12.589,2.046)--
(12.597,2.053)--
(12.605,2.079)--
(12.614,2.071)--
(12.622,2.103)--
(12.63,2.184)--
(12.638,2.013)--
(12.647,2.011)--
(12.655,2.085)--
(12.663,2.039)--
(12.671,2.008)--
(12.679,2.024)--
(12.688,2.05)--
(12.696,2.049)--
(12.704,2.07)--
(12.712,2.078)--
(12.721,2.103)--
(12.729,2.089)--
(12.737,2.089)--
(12.745,2.097)--
(12.753,2.11)--
(12.762,2.114)--
(12.77,2.082)--
(12.778,2.086)--
(12.786,2.079)--
(12.795,2.079)--
(12.803,2.074)--
(12.811,2.079)--
(12.819,2.045)--
(12.827,2.039)--
(12.836,2.052)--
(12.844,2.029)--
(12.852,2.05)--
(12.86,2.04)--
(12.868,2.046)--
(12.877,2.072)--
(12.885,2.072)--
(12.893,2.089)--
(12.901,2.1)--
(12.91,2.094)--
(12.918,2.103)--
(12.926,2.113)--
(12.934,2.136)--
(12.942,2.132)--
(12.951,2.14)--
(12.959,2.136)--
(12.967,2.127)--
(12.975,2.133)--
(12.984,2.129)--
(12.992,2.135)--
(13,2.133)--
(13.005,2.129)--
(13.014,2.131)--
(13.022,2.142)--
(13.03,2.157)--
(13.038,2.161)--
(13.047,2.204)--
(13.055,2.23)--
(13.063,2.283)--
(13.071,2.255)--
(13.079,2.294)--
(13.088,2.324)--
(13.096,2.318)--
(13.104,2.345)--
(13.112,2.384)--
(13.121,2.424)--
(13.129,2.408)--
(13.137,2.474)--
(13.145,2.467)--
(13.153,2.494)--
(13.162,2.543)--
(13.17,2.561)--
(13.178,2.628)--
(13.186,2.667)--
(13.195,2.67)--
(13.203,2.673)--
(13.211,2.762)--
(13.219,2.854)--
(13.227,2.869)--
(13.236,2.971)--
(13.244,2.966)--
(13.252,3.142)--
(13.26,3.154)--
(13.268,3.377)--
(13.277,2.884)--
(13.285,2.959)--
(13.293,2.985)--
(13.301,3.097)--
(13.31,3.185)--
(13.318,3.107)--
(13.326,3.143)--
(13.334,2.969)--
(13.342,3.083)--
(13.351,3.04)--
(13.359,3.058)--
(13.367,3.061)--
(13.375,3.093)--
(13.384,3.088)--
(13.392,3.119)--
(13.4,3.123)--
(13.408,3.117)--
(13.416,3.081)--
(13.425,3.088)--
(13.433,3.033)--
(13.441,3.033)--
(13.449,3)--
(13.458,3.002)--
(13.466,3.049)--
(13.474,3.032)--
(13.482,3.019)--
(13.49,2.982)--
(13.499,2.952)--
(13.507,2.832)--
(13.515,2.89)--
(13.523,2.94)--
(13.532,2.977)--
(13.54,2.991)--
(13.548,2.963)--
(13.556,2.98)--
(13.564,2.984)--
(13.573,3.005)--
(13.581,3.018)--
(13.589,3.02)--
(13.597,3.024)--
(13.605,3.011)--
(13.614,3.031)--
(13.622,2.993)--
(13.63,3.009)--
(13.638,3.045)--
(13.647,3.053)--
(13.655,3.076)--
(13.663,3.123)--
(13.671,3.115)--
(13.679,3.088)--
(13.688,3.085)--
(13.696,3.109)--
(13.704,3.099)--
(13.712,3.105)--
(13.721,3.092)--
(13.729,3.088)--
(13.737,3.099)--
(13.745,3.1)--
(13.753,3.068)--
(13.762,3.085)--
(13.77,3.101)--
(13.778,3.106)--
(13.786,3.144)--
(13.795,3.178)--
(13.803,3.248)--
(13.811,3.292)--
(13.819,3.277)--
(13.827,3.308)--
(13.836,3.31)--
(13.844,3.392)--
(13.852,3.513)--
(13.86,3.531)--
(13.868,3.62)--
(13.877,3.666)--
(13.885,3.775)--
(13.893,3.923)--
(13.901,3.927)--
(13.91,4.035)--
(13.918,3.997)--
(13.926,4.012)--
(13.934,3.859)--
(13.942,3.948)--
(13.951,3.937)--
(13.959,3.846)--
(13.967,3.82)--
(13.975,3.806)--
(13.984,3.866)--
(13.992,3.854)--
(14,3.873)--
(14.008,3.915)--
(14.016,3.938)--
(14.025,3.918)--
(14.033,3.907)--
(14.041,3.92)--
(14.049,3.921)--
(14.058,3.91)--
(14.066,3.906)--
(14.074,3.903)--
(14.082,3.904)--
(14.09,3.911)--
(14.099,3.891)--
(14.107,3.851)--
(14.115,3.824)--
(14.123,3.814)--
(14.132,3.797)--
(14.14,3.753)--
(14.148,3.736)--
(14.156,3.767)--
(14.164,3.748)--
(14.173,3.823)--
(14.181,3.785)--
(14.189,3.794)--
(14.197,3.804)--
(14.205,3.796)--
(14.214,3.771)--
(14.222,3.754)--
(14.23,3.768)--
(14.238,3.699)--
(14.247,3.681)--
(14.255,3.649)--
(14.263,3.651)--
(14.271,3.603)--
(14.279,3.607)--
(14.288,3.709)--
(14.296,3.699)--
(14.304,3.693)--
(14.312,3.662)--
(14.321,3.65)--
(14.329,3.663)--
(14.337,3.64)--
(14.345,3.65)--
(14.353,3.656)--
(14.362,3.642)--
(14.37,3.653)--
(14.378,3.65)--
(14.386,3.719)--
(14.395,3.76)--
(14.403,3.759)--
(14.411,3.793)--
(14.419,3.829)--
(14.427,3.817)--
(14.436,3.814)--
(14.444,3.79)--
(14.452,3.749)--
(14.46,3.781)--
(14.468,3.772)--
(14.477,3.768)--
(14.485,3.77)--
(14.493,3.792)--
(14.501,3.809)--
(14.51,3.802)--
(14.518,3.796)--
(14.526,3.801)--
(14.534,3.795)--
(14.542,3.799)--
(14.551,3.792)--
(14.559,3.779)--
(14.567,3.773)--
(14.575,3.759)--
(14.584,3.772)--
(14.592,3.764)--
(14.6,3.77)--
(14.608,3.763)--
(14.616,3.717)--
(14.625,3.692)--
(14.633,3.705)--
(14.641,3.702)--
(14.649,3.71)--
(14.658,3.709)--
(14.666,3.684)--
(14.674,3.687)--
(14.682,3.682)--
(14.69,3.686)--
(14.699,3.681)--
(14.707,3.67)--
(14.715,3.601)--
(14.723,3.603)--
(14.732,3.611)--
(14.74,3.58)--
(14.748,3.586)--
(14.756,3.526)--
(14.764,3.519)--
(14.773,3.555)--
(14.781,3.581)--
(14.789,3.578)--
(14.797,3.59)--
(14.805,3.586)--
(14.814,3.543)--
(14.822,3.55)--
(14.83,3.533)--
(14.838,3.513)--
(14.847,3.542)--
(14.855,3.552)--
(14.863,3.634)--
(14.871,3.572)--
(14.879,3.58)--
(14.888,3.553)--
(14.896,3.584)--
(14.904,3.571)--
(14.912,3.575)--
(14.921,3.578)--
(14.929,3.573)--
(14.937,3.544)--
(14.945,3.55)--
(14.953,3.547)--
(14.962,3.502)--
(14.97,3.514)--
(14.978,3.515)--
(14.986,3.498)--
(14.995,3.496)--
(15.003,3.5)--
(15.011,3.442)--
(15.019,3.442)--
(15.027,3.435)--
(15.036,3.247)--
(15.044,3.295)--
(15.052,3.328)--
(15.06,3.367)--
(15.068,3.434)--
(15.077,3.368)--
(15.085,3.344)--
(15.093,3.347)--
(15.101,3.352)--
(15.11,3.343)--
(15.118,3.38)--
(15.126,3.373)--
(15.134,3.383)--
(15.142,3.373)--
(15.151,3.378)--
(15.159,3.403)--
(15.167,3.441)--
(15.175,3.435)--
(15.184,3.459)--
(15.192,3.473)--
(15.2,3.453)--
(15.208,3.425)--
(15.216,3.411)--
(15.225,3.394)--
(15.233,3.396)--
(15.241,3.389)--
(15.249,3.402)--
(15.258,3.41)--
(15.266,3.391)--
(15.274,3.374)--
(15.282,3.334)--
(15.29,3.348)--
(15.299,3.351)--
(15.307,3.372)--
(15.315,3.339)--
(15.323,3.354)--
(15.332,3.369)--
(15.34,3.37)--
(15.348,3.389)--
(15.356,3.388)--
(15.364,3.377)--
(15.373,3.373)--
(15.381,3.37)--
(15.389,3.378)--
(15.397,3.373)--
(15.405,3.373)--
(15.414,3.347)--
(15.422,3.353)--
(15.43,3.348)--
(15.438,3.358)--
(15.447,3.362)--
(15.455,3.39)--
(15.463,3.392)--
(15.471,3.392)--
(15.479,3.384)--
(15.488,3.396)--
(15.496,3.411)--
(15.504,3.411)--
(15.512,3.427)--
(15.521,3.458)--
(15.529,3.462)--
(15.537,3.441)--
(15.545,3.441)--
(15.553,3.443)--
(15.562,3.458)--
(15.57,3.47)--
(15.578,3.455)--
(15.586,3.454)--
(15.595,3.443)--
(15.603,3.424)--
(15.611,3.428)--
(15.619,3.424)--
(15.627,3.405)--
(15.636,3.368)--
(15.644,3.329)--
(15.652,3.358)--
(15.66,3.355)--
(15.668,3.363)--
(15.677,3.37)--
(15.685,3.386)--
(15.693,3.38)--
(15.701,3.363)--
(15.71,3.369)--
(15.718,3.362)--
(15.726,3.362)--
(15.734,3.369)--
(15.742,3.376)--
(15.751,3.376)--
(15.759,3.379)--
(15.767,3.387)--
(15.775,3.395)--
(15.784,3.406)--
(15.792,3.43)--
(15.8,3.431)--
(15.808,3.443)--
(15.816,3.455)--
(15.825,3.492)--
(15.833,3.493)--
(15.841,3.641)--
(15.849,3.588)--
(15.858,3.548)--
(15.866,3.521)--
(15.874,3.518)--
(15.882,3.517)--
(15.89,3.508)--
(15.899,3.512)--
(15.907,3.549)--
(15.915,3.555)--
(15.923,3.557)--
(15.932,3.597)--
(15.94,3.619)--
(15.948,3.642)--
(15.956,3.657)--
(15.964,3.664)--
(15.973,3.639)--
(15.981,3.658)--
(15.989,3.627)--
(15.997,3.633)--
(16.005,3.632)--
(16.014,3.634)--
(16.022,3.653)--
(16.03,3.65)--
(16.038,3.593)--
(16.047,3.586)--
(16.055,3.611)--
(16.063,3.607)--
(16.071,3.596)--
(16.079,3.578)--
(16.088,3.572)--
(16.096,3.587)--
(16.104,3.575)--
(16.112,3.576)--
(16.121,3.605)--
(16.129,3.621)--
(16.137,3.643)--
(16.145,3.62)--
(16.153,3.628)--
(16.162,3.64)--
(16.17,3.625)--
(16.178,3.612)--
(16.186,3.616)--
(16.195,3.613)--
(16.203,3.618)--
(16.211,3.612)--
(16.219,3.613)--
(16.227,3.62)--
(16.236,3.63)--
(16.244,3.615)--
(16.252,3.621)--
(16.26,3.625)--
(16.268,3.626)--
(16.277,3.624)--
(16.285,3.627)--
(16.293,3.629)--
(16.301,3.646)--
(16.31,3.654)--
(16.318,3.67)--
(16.326,3.659)--
(16.334,3.647)--
(16.342,3.652)--
(16.351,3.661)--
(16.359,3.656)--
(16.367,3.659)--
(16.375,3.656)--
(16.384,3.645)--
(16.392,3.646)--
(16.4,3.656)--
(16.408,3.709)--
(16.416,3.732)--
(16.425,3.759)--
(16.433,3.762)--
(16.441,3.762)--
(16.449,3.846)--
(16.458,3.882)--
(16.466,3.881)--
(16.474,3.769)--
(16.482,3.823)--
(16.49,3.81)--
(16.499,3.829)--
(16.507,3.83)--
(16.515,3.804)--
(16.523,3.812)--
(16.532,3.818)--
(16.54,3.821)--
(16.548,3.828)--
(16.556,3.814)--
(16.564,3.816)--
(16.573,3.816)--
(16.581,3.798)--
(16.589,3.752)--
(16.597,3.77)--
(16.605,3.77)--
(16.614,3.769)--
(16.622,3.756)--
(16.63,3.76)--
(16.638,3.766)--
(16.647,3.766)--
(16.655,3.757)--
(16.663,3.762)--
(16.671,3.761)--
(16.679,3.784)--
(16.688,3.798)--
(16.696,3.784)--
(16.704,3.787)--
(16.712,3.784)--
(16.721,3.785)--
(16.729,3.781)--
(16.737,3.784)--
(16.745,3.783)--
(16.753,3.786)--
(16.762,3.787)--
(16.77,3.791)--
(16.778,3.806)--
(16.786,3.806)--
(16.795,3.805)--
(16.803,3.799)--
(16.811,3.815)--
(16.819,3.828)--
(16.827,3.854)--
(16.836,3.862)--
(16.844,3.847)--
(16.852,3.847)--
(16.86,3.854)--
(16.868,3.846)--
(16.877,3.867)--
(16.885,3.875)--
(16.893,3.874)--
(16.901,3.869)--
(16.91,3.865)--
(16.918,3.876)--
(16.926,3.884)--
(16.934,3.884)--
(16.942,3.888)--
(16.951,3.891)--
(16.959,3.893)--
(16.967,3.897)--
(16.975,3.935)--
(16.984,3.948)--
(16.992,3.986)--
(17,3.982)--
(17.005,4.01)--
(17.014,3.946)--
(17.022,3.951)--
(17.03,3.905)--
(17.038,3.915)--
(17.047,3.942)--
(17.055,3.964)--
(17.063,3.95)--
(17.071,3.963)--
(17.079,3.964)--
(17.088,4.003)--
(17.096,4.006)--
(17.104,4.022)--
(17.112,4.004)--
(17.121,4.005)--
(17.129,4.023)--
(17.137,4.035)--
(17.145,4.069)--
(17.153,4.07)--
(17.162,4.087)--
(17.17,4.103)--
(17.178,4.093)--
(17.186,4.041)--
(17.195,4.093)--
(17.203,4.072)--
(17.211,4.013)--
(17.219,4.012)--
(17.227,3.982)--
(17.236,4.02)--
(17.244,4.033)--
(17.252,4.058)--
(17.26,4.078)--
(17.268,4.082)--
(17.277,4.086)--
(17.285,4.074)--
(17.293,4.085)--
(17.301,4.1)--
(17.31,4.101)--
(17.318,4.129)--
(17.326,4.131)--
(17.334,4.178)--
(17.342,4.193)--
(17.351,4.236)--
(17.359,4.236)--
(17.367,4.236)--
(17.375,4.279)--
(17.384,4.311)--
(17.392,4.376)--
(17.4,4.304)--
(17.408,4.35)--
(17.416,4.388)--
(17.425,4.431)--
(17.433,4.446)--
(17.441,4.472)--
(17.449,4.389)--
(17.458,4.426)--
(17.466,4.44)--
(17.474,4.433)--
(17.482,4.387)--
(17.49,4.406)--
(17.499,4.398)--
(17.507,4.418)--
(17.515,4.409)--
(17.523,4.375)--
(17.532,4.341)--
(17.54,4.338)--
(17.548,4.462)--
(17.556,4.435)--
(17.564,4.397)--
(17.573,4.435)--
(17.581,4.433)--
(17.589,4.458)--
(17.597,4.532)--
(17.605,4.535)--
(17.614,4.615)--
(17.622,4.64)--
(17.63,4.626)--
(17.638,4.611)--
(17.647,4.64)--
(17.655,4.643)--
(17.663,4.677)--
(17.671,4.667)--
(17.679,4.667)--
(17.688,4.641)--
(17.696,4.625)--
(17.704,4.577)--
(17.712,4.612)--
(17.721,4.563)--
(17.729,4.569)--
(17.737,4.624)--
(17.745,4.637)--
(17.753,4.633)--
(17.762,4.638)--
(17.77,4.679)--
(17.778,4.726)--
(17.786,4.752)--
(17.795,4.744)--
(17.803,4.78)--
(17.811,4.741)--
(17.819,4.761)--
(17.827,4.786)--
(17.836,4.849)--
(17.844,4.868)--
(17.852,4.87)--
(17.86,4.804)--
(17.868,4.822)--
(17.877,4.891)--
(17.885,4.917)--
(17.893,4.911)--
(17.901,4.968)--
(17.91,4.995)--
(17.918,5.044)--
(17.926,5.075)--
(17.934,5.204)--
(17.942,5.224)--
(17.951,5.222)--
(17.959,5.285)--
(17.967,5.205)--
(17.975,5.186)--
(17.984,5.204)--
(17.992,5.166)--
(18,5.14)--
(18.008,5.182)--
(18.016,5.221)--
(18.025,5.18)--
(18.033,5.161)--
(18.041,5.048)--
(18.049,5.058)--
(18.058,5.023)--
(18.066,5.05)--
(18.074,5.071)--
(18.082,5.005)--
(18.09,4.958)--
(18.099,4.886)--
(18.107,4.931)--
(18.115,4.945)--
(18.123,4.999)--
(18.132,5.021)--
(18.14,5.023)--
(18.148,4.987)--
(18.156,5.032)--
(18.164,5.044)--
(18.173,5.064)--
(18.181,4.974)--
(18.189,4.99)--
(18.197,4.911)--
(18.205,4.903)--
(18.214,4.954)--
(18.222,4.939)--
(18.23,4.914)--
(18.238,4.856)--
(18.247,4.832)--
(18.255,4.832)--
(18.263,4.841)--
(18.271,4.832)--
(18.279,4.897)--
(18.288,4.905)--
(18.296,4.917)--
(18.304,4.946)--
(18.312,4.954)--
(18.321,4.97)--
(18.329,4.958)--
(18.337,4.987)--
(18.345,4.971)--
(18.353,4.959)--
(18.362,4.941)--
(18.37,4.921)--
(18.378,4.915)--
(18.386,4.904)--
(18.395,4.872)--
(18.403,4.853)--
(18.411,4.875)--
(18.419,4.886)--
(18.427,4.884)--
(18.436,4.879)--
(18.444,4.815)--
(18.452,4.808)--
(18.46,4.827)--
(18.468,4.828)--
(18.477,4.781)--
(18.485,4.786)--
(18.493,4.805)--
(18.501,4.82)--
(18.51,4.818)--
(18.518,4.828)--
(18.526,4.795)--
(18.534,4.801)--
(18.542,4.869)--
(18.551,4.866)--
(18.559,4.909)--
(18.567,4.904)--
(18.575,4.911)--
(18.584,4.88)--
(18.592,4.845)--
(18.6,4.81)--
(18.608,4.792)--
(18.616,4.782)--
(18.625,4.811)--
(18.633,4.809)--
(18.641,4.809)--
(18.649,4.824)--
(18.658,4.848)--
(18.666,4.851)--
(18.674,4.865)--
(18.682,4.809)--
(18.69,4.799)--
(18.699,4.81)--
(18.707,4.812)--
(18.715,4.802)--
(18.723,4.827)--
(18.732,4.807)--
(18.74,4.825)--
(18.748,4.819)--
(18.756,4.817)--
(18.764,4.817)--
(18.773,4.817)--
(18.781,4.797)--
(18.789,4.819)--
(18.797,4.812)--
(18.805,4.813)--
(18.814,4.811)--
(18.822,4.809)--
(18.83,4.8)--
(18.838,4.804)--
(18.847,4.809)--
(18.855,4.807)--
(18.863,4.806)--
(18.871,4.749)--
(18.879,4.749)--
(18.888,4.656)--
(18.896,4.633)--
(18.904,4.574)--
(18.912,4.614)--
(18.921,4.599)--
(18.929,4.573)--
(18.937,4.548)--
(18.945,4.539)--
(18.953,4.509)--
(18.962,4.552)--
(18.97,4.604)--
(18.978,4.621)--
(18.986,4.574)--
(18.995,4.584)--
(19.003,4.587)--
(19.011,4.588)--
(19.019,4.606)--
(19.027,4.563)--
(19.036,4.557)--
(19.044,4.559)--
(19.052,4.559)--
(19.06,4.554)--
(19.068,4.555)--
(19.077,4.534)--
(19.085,4.538)--
(19.093,4.538)--
(19.101,4.532)--
(19.11,4.562)--
(19.118,4.559)--
(19.126,4.56)--
(19.134,4.595)--
(19.142,4.599)--
(19.151,4.583)--
(19.159,4.585)--
(19.167,4.583)--
(19.175,4.587)--
(19.184,4.593)--
(19.192,4.589)--
(19.2,4.593)--
(19.208,4.602)--
(19.216,4.605)--
(19.225,4.602)--
(19.233,4.603)--
(19.241,4.614)--
(19.249,4.67)--
(19.258,4.697)--
(19.266,4.717)--
(19.274,4.709)--
(19.282,4.706)--
(19.29,4.717)--
(19.299,4.725)--
(19.307,4.743)--
(19.315,4.723)--
(19.323,4.722)--
(19.332,4.73);
